Explicitly capturing demonstrator multi-modality for distillation into diffusion policies

The diversity of a distilled diffusion policy's outputs matters beyond how it impacts the policy's success rate. In particular, downstream applications like test-time search and policy improvement require exploration. Thus, we want to distill multi-modal demonstrators into diffusion policies which reproduce their conditional action distributions. Standard data collection for behavior cloning applies a sliding window to demonstration episodes, which pairs unique observation histories with actions. These datasets can be fit by a policy that is either multi-modal, or unimodal with high Lipschitz constant to capture a diversity of actions seen at nearby observation samples. Prior work finds that diffusion policies trained on sparse data learn the latter, memorizing one action per observation. We adapt vine sampling to behavior cloning data collection to resolve this ambiguity: at some states the demonstrator visits, query it $k$ times from exactly the same observation. On a synthetic task, we study how the number of actions per observation, $k$, affects the learned policy, and find that larger $k$ yields a policy that better matches the demonstrator's conditional distribution, including its multi-modality and diversity. On a 2D truck unloading task, vine sampling likewise leads to a policy closer to the demonstrator and substantially improves both best-of-$N$ and expert iteration performance.

==> preamble.tex <==
\makeatletter
\newif\ifcorl
\@ifpackageloaded{corl_2026}{\corltrue}{\corlfalse}
\makeatother

\usepackage[utf8]{inputenc}      %
\usepackage[T1]{fontenc}         %
\usepackage{microtype}           %
\usepackage{textcomp}            %

\usepackage{amsmath, amssymb, amsfonts, amsthm, mathtools}
\usepackage{bm}                  %
\usepackage{dsfont}              %
\usepackage{nicefrac}

\usepackage{graphicx}
\usepackage{booktabs}
\usepackage{subcaption}
\usepackage{xcolor}

\ifcorl
  \captionsetup{font=small}
\else
  \captionsetup{font=small, skip=3pt}
\fi
\captionsetup[figure]{name=Fig.}

\makeatletter
\newcommand{\sublabel}[1]{%
  \refstepcounter{subfigure}%
  \@ifundefined{hc@currentHref}{}{\let\@currentHref\hc@currentHref}%
  \label{#1}}
\makeatother

\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=1.18}
\usetikzlibrary{arrows.meta, positioning, calc, fit, shapes.geometric}

\usepackage[ruled,linesnumbered]{algorithm2e}
\usepackage{wrapfig}

\setlength{\textfloatsep}{8pt plus 2pt minus 2pt}   %
\setlength{\floatsep}{6pt plus 2pt minus 2pt}       %
\setlength{\intextsep}{6pt plus 2pt minus 2pt}      %
\ifcorl\else
\setlength{\abovedisplayskip}{4pt plus 2pt minus 2pt}
\setlength{\belowdisplayskip}{4pt plus 2pt minus 2pt}
\setlength{\abovedisplayshortskip}{0pt plus 2pt}
\setlength{\belowdisplayshortskip}{2pt plus 2pt minus 2pt}
\setlength{\parskip}{6pt}
\makeatletter
\def\section{\@startsection{section}{1}{\z@}{-1.4ex plus -0.4ex minus -.2ex}%
  {0.9ex plus 0.2ex minus 0.1ex}{\large\sc\raggedright}}
\def\subsection{\@startsection{subsection}{2}{\z@}{-1.2ex plus -0.4ex minus -.2ex}%
  {0.5ex plus .1ex}{\normalsize\sc\raggedright}}
\def\subsubsection{\@startsection{subsubsection}{3}{\z@}{-1.0ex plus -0.3ex minus -.2ex}%
  {0.3ex plus .1ex}{\normalsize\sc\raggedright}}
\makeatother
\fi %

\usepackage{enumitem}
\ifcorl\else %
\setlist{itemsep=2pt, topsep=2pt}
\fi

\ifcorl\else
\usepackage[colorlinks=true,
            linkcolor=blue!50!black,
            citecolor=blue!50!black,
            urlcolor=blue!60!black]{hyperref}
\fi
\usepackage{url}
\usepackage[all]{hypcap}

\makeatletter
\newcommand{\algtop}{\phantomsection\global\let\alg@topHref\@currentHref}
\newcommand{\alglabel}[1]{%
  \@ifundefined{alg@topHref}{}{\let\@currentHref\alg@topHref}%
  \label{#1}}
\makeatother

\usepackage{cleveref}

\crefname{figure}{fig.}{figs.}        \Crefname{figure}{Fig.}{Figs.}
\crefname{subfigure}{fig.}{figs.}     \Crefname{subfigure}{Fig.}{Figs.}
\crefname{equation}{eq.}{eqs.}        \Crefname{equation}{Eq.}{Eqs.}
\crefname{algorithm}{alg.}{algs.}     \Crefname{algorithm}{Alg.}{Algs.}
\crefname{section}{sec.}{secs.}       \Crefname{section}{Sec.}{Secs.}
\crefname{appendix}{app.}{apps.}      \Crefname{appendix}{App.}{Apps.}
\crefname{subappendix}{app.}{apps.}   \Crefname{subappendix}{App.}{Apps.}
\crefname{subsubappendix}{app.}{apps.} \Crefname{subsubappendix}{App.}{Apps.}
\crefname{definition}{def.}{defs.}    \Crefname{definition}{Def.}{Defs.}
\crefname{table}{table}{tables}       \Crefname{table}{Table}{Tables}

\setlength{\marginparwidth}{2cm}
\usepackage[textsize=footnotesize]{todonotes}
\setuptodonotes{inline}

\usepackage[draft, commentmarkup=todo, authormarkup=none]{changes}
\definechangesauthor[name={Shao Yuan Chew Chia}, color=magenta!70!black]{SY}
\definechangesauthor[name={Abhinav Agarwal},color=blue]{AA}
\definechangesauthor[name={Rebecca H. Jiang}, color=teal!80!black]{RJ}

\newcommand{\sycomment}[1]{\comment[id=SY]{#1}}
\newcommand{\syadded}[1]{\added[id=SY]{#1}}
\newcommand{\sydeleted}[1]{\deleted[id=SY]{#1}}
\newcommand{\syreplaced}[2]{\replaced[id=SY]{#1}{#2}}

\newcommand{\aacomment}[1]{\comment[id=AA]{#1}}
\newcommand{\rjcomment}[1]{\comment[id=RJ]{#1}}

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{example}[theorem]{Example}
\newtheorem{problem}[theorem]{Problem}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

\crefname{assumption}{Assumption}{Assumptions}
\crefname{problem}{Problem}{Problems}

